BONES: Near-Optimal Neural-Enhanced Video Streaming

Accessing high-quality video content can be challenging due to insufficient and unstable network bandwidth. Recent advances in neural enhancement have shown promising results in improving the quality of degraded videos through deep learning. Neural-Enhanced Streaming (NES) incorporates this new approach into video streaming, allowing users to download low-quality video segments and then enhance them to obtain high-quality content without violating the playback of the video stream. We introduce BONES, an NES control algorithm that jointly manages the network and computational resources to maximize the quality of experience (QoE) of the user. BONES formulates NES as a Lyapunov optimization problem and solves it in an online manner with near-optimal performance, making it the first NES algorithm to provide a theoretical performance guarantee. Comprehensive experimental results indicate that BONES increases QoE by 5\% to 20\% over state-of-the-art algorithms with minimal overhead. Our code is available at https://github.com/UMass-LIDS/bones.

==> backup.tex <==

Review \#69A
===========================================================================

Overall merit
-------------
4. Strong accept (top 5%)

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
This paper addresses the problem of enhancing the user’s Quality of Experience in video streaming applications. Specifically, the authors consider the problem of joint control of download bitrate and video enhancement mechanism. The authors address the problem using a Lyapunov Optimization approach, which allows them to obtain performance guarantees for their algorithm, denoted BONES. The authors provide extensive evaluation and comparison with state of the art.

Strengths
---------
- This is an important topic. As the authors mention, the majority of the internet traffic is video and this trend may continue in the future. Hence, coming up with strategies to improve QoE is critical.

- The authors leverage a traditional technique (Lyapunov Optimization) to address this modern problem in a unique way. I appreciate the authors effort to prove that BONES does not violate queueing capacity and can achieve near-optimal performance. I also find the mathematical model utilized by the authors very interesting.

- In addition to the theoretical contributions, the authors provide a comprehensive evaluation of BONES, comparing it with (several) state-of-the-art ABR and NES algorithms.

Weaknesses
----------
- Prior work on ABR algorithms often leverages methods such as Machine Learning and Model Predictive Control to predict future available bandwidth and act preemptively. In contrast, BONES uses a Greedy-like myopic approach that only takes the current queue-length (and some static information) into consideration when making decisions. In fact, the only source of randomness in the optimization problem is the current network bandwidth w(t), which is omitted in (11), making it a deterministic problem. My concern is twofold: (1) How come BONES outperforms predictive algorithms such as Pensieve? I understand that Pensieve (with Greedy enhancements) does not make joint bandwidth and enhancement decisions, but it does attempt to take the future into account (which BONES doesn’t). If Pensieve (or any other predictive algorithm) had perfect information about the future, would it (significantly) outperform BONES? (2) Would it be possible to incorporate prediction into BONES? Perhaps with loss of performance guarantee?

- The authors discuss three important basic QoE metrics, namely visual quality (VMAF), quality oscillation (VMAF), and rebuffering rate (%). Then, the authors define a composite QoE. From Table 4, it seems that Pensieve always has the best visual quality, FastMPC always has the best quality oscillation, and Throughput always has the best rebuffering rate. It seems that BONES only outperforms the state of the art in the composite QoE. I wonder how much of the performance improvement achieved by BONES is due to this particular definition of QoE. Are there other reasonable composite QoE metrics widely used? If so, it would be interesting to see a comparison.

- I am not convinced that maximizing \bar_s, defined in (5), is equivalent to minimizing the total rebuffering time. This may need a much more detailed argument.

- Minor question: Do we need ej in eq (5)?



Review \#69B
===========================================================================

Overall merit
-------------
3. Accept (5-15%)

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper proposes Buffer-Occupancy-based Neural-Enhanced Streaming (BONES), a client-side Neural-Enhanced Streaming (NES) algorithm that addresses the challenges of delivering high-quality video content over the internet in the face of limited and unstable network bandwidth. While traditional Adaptive Bitrate (ABR) algorithms adjust video quality based on available bandwidth, BONES introduces a novel approach that incorporates client-side video quality enhancement options obtained using machine learning (with different computational requirements). This allows for a tradeoff between communication and computational resources and overcomes limitations of prior NES methods. BONES offers provable performance guarantees and a simple design, outperforming existing methods in experimental tests and demonstrating significant Quality of Experience (QoE) improvements with low overhead.

Strengths
---------
+ Well-motivated and natural extension to prior work, resulting in a surprisingly simple and efficient algorithm

+ Solution provides theoretic guarantees

+ Provide clear insights into the best choices and the impact of parameters

+ Appears to be relatively practical

+ Shown to outperform prior works, backed up with experiments and comparisons against prior works

+ Appears to be first to consider non-real-time enhancements and buffer of computations.  (Think more can be done here, but by sharing code, hopefully will allow others to build on the work.)

Weaknesses
----------
- The paper leaves many open aspects, including how to find a good balance and delivery of the enhancement models (e.g., content-aware vs content-agnostic), and several aspects left as future work (e.g., see end of conclusions).

- It is unclear how realistic scenarios the system is evaluated on and the performance for the network-traces were not that convincing.  This leaves several question marks regarding to what extent the method would provide improvements in practice.

- It is also unclear how practical the application would be (e.g., clients that have very poor connection but powerful computers ...) or whether the paper addresses a corner case.  In practice, I am worried that regular HAS/DASH will be good enough for most practical purposes.

- It would be valuable to discuss the data requirements and potential limitations of BONES, especially in terms of data collection and computational resources needed for training (and who does the training when).  Some additional motivation may also be needed to motivate this use case in practice.  As of now, it is not obvious how and what incentives there are to deploy and integrate BONES into existing video streaming systems.

Comments for authors
--------------------
Additional comments:
- still unsure if I am okay with the first sentence ...
- would be good to say what type of guarantees (in the abstract)
- I did not like how many of the equations were introduced (e.g., equations (4) and (5).  I would have much rather seen them integrated into the text (e.g., as equations (6), (7), and (8)).
+ really like Figure 2
- Please sort out y-axes numbering in Figure 6 (would not rotate these numbers)
- Results in Figure 5 (and some others) may be made to be easier to
- Would be nice to see more details/data regarding the increase in startup due to use of content-aware enhancement



Review \#69C
===========================================================================

Overall merit
-------------
2. Reject (15-30%)

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper introduced BONES, which jointly manages network and computational resources to maximize QoE of users. The algorithm formulates the streaming problem as a Lyapunov optimization problem and offers online solution for it. Experimental results show that BONES improves QoE compared to baselines.

Strengths
---------
- The paper is in general well written. The formulation is clearly presented and the algorithm is explained with sufficient detail. The use of Lyapunov optimization is also clearly explained.

Weaknesses
----------
- There have been more recent DRL solutions for scheduling problems. It would be helpful to use some of them as baselines. Right now the baselines are not the most recent algorithms (except only for PreSR).
- My main concern of the paper would be about its contribution. First of all, the application of the Lyapunov optimization technique is quite standard. Thus, the theoretical contribution is limited. On the other hand, the experiments are done mainly by simulation (based on real traces). Although the comparison appears comprehensive, it would be better to have some test on real testbed.

Comments for authors
--------------------
- There have been more recent DRL solutions for scheduling problems. It would be helpful to use some of them as baselines. Right now the baselines are not the most recent algorithms (except only for PreSR).
- My main concern of the paper would be about its contribution. First of all, the application of the Lyapunov optimization technique is quite standard. Thus, the theoretical contribution is limited. On the other hand, the experiments are done mainly by simulation (based on real traces). Although the comparison appears comprehensive, it would be better to have some test on real testbed.





==> revision.tex <==
\section{One-Shot Revision Summary}

% \textbf{Paper:} BONES: Near-Optimal Neural-Enhanced Video Streaming

We are grateful to the reviewers for their valuable feedback and insight. In the text below, we have summarized all revision requests and additional comments from the reviewers, along with our responses.

% We have addressed all of the revision requests and additional comments from the reviewers. And we provide a summary below.

\textbf{Meta-review:} \textit{In summary, the TPC members concluded that the main strengths of this paper are: its focus on an important and relevant problem; its theoretical guarantees; outperforming prior work in simulations. The major concern is whether the improvements obtained in simulations will translate to practice. It is important to emphasize the prior work has leveraged (prototype) system implementations to compare their solutions with the state-of-the-art. To address this major concern, we request that the authors implement BONES and a few state-of-the-art systems and compare them in real-world scenarios.}

\textbf{Revision Request:} \textit{Implement a prototype system of \bones and compare it with state-of-the-art methods in real-world scenarios. }

\rev{In response to the revision request, we have implemented a prototype system within which we have compared \bones with other state-of-the-art methods in field tests. We presented a detailed introduction to the system structure, experimental settings, and result analysis in \cref{sec:prototype}. According to the experimental results, we conclude that the advantages of \bones not only hold in large-scale simulations but also translate to real-world scenarios. We will release our system prototype and codes to the public. Additionally, we extend the overhead analysis in \cref{sec:overhead} as required by reviewers. We introduce a new heuristic to eliminate the startup latency of neural enhancement, and provide three trade-offs between overhead and performance. }

% \hrulefill

In the following, we also respond to the reviewers' additional requests and comments.

% - Prior work on ABR algorithms often leverages methods such as Machine Learning and Model Predictive Control to predict future available bandwidth and act preemptively. In contrast, BONES uses a Greedy-like myopic approach that only takes the current queue-length (and some static information) into consideration when making decisions. In fact, the only source of randomness in the optimization problem is the current network bandwidth w(t), which is omitted in (11), making it a deterministic problem. My concern is twofold: (1) How come BONES outperforms predictive algorithms such as Pensieve? I understand that Pensieve (with Greedy enhancements) does not make joint bandwidth and enhancement decisions, but it does attempt to take the future into account (which BONES doesn’t). If Pensieve (or any other predictive algorithm) had perfect information about the future, would it (significantly) outperform BONES? (2) Would it be possible to incorporate prediction into BONES? Perhaps with loss of performance guarantee?

% - The authors discuss three important basic QoE metrics, namely visual quality (VMAF), quality oscillation (VMAF), and rebuffering rate. Then, the authors define a composite QoE. From Table 4, it seems that Pensieve always has the best visual quality, FastMPC always has the best quality oscillation, and Throughput always has the best rebuffering rate. It seems that BONES only outperforms the state of the art in the composite QoE. I wonder how much of the performance improvement achieved by BONES is due to this particular definition of QoE. Are there other reasonable composite QoE metrics widely used? If so, it would be interesting to see a comparison.

% - I am not convinced that maximizing $\bar_s$, defined in (5), is equivalent to minimizing the total rebuffering time. This may need a much more detailed argument.

% - Minor question: Do we need ej in eq (5)?

\textbf{Review \#69A:} \textit{Why \bones can outperform predictive algorithms that consider future bandwidth variation? Will predictive algorithms outperform \bones with perfect information about the future? Is it possible to incorporate prediction into \bones?}

%  They are especially fragile to abrupt bandwidth changes like those in \cref{fig:istream}.
\rev{The reasons why \bones can outperform algorithms considering future bandwidth are as follows: (1) Perfect prediction doesn't exist. Most studies adopt simple prediction methods such as exponential or geometric averages, while a few others use more complex RL methods. However, no method can perfectly capture the highly dynamic and heavy-tailed real-world scenarios. (2) Even with perfect knowledge about the future, it's computationally expensive to utilize it optimally. Given future bandwidth information (even over a short period), it requires solving a Model Predictive Control or Dynamic Programming problem to find the optimal solution, which is infeasible in practice. As a result, PreSR \cite{presr} relies on a sub-optimal heuristic search, Pensieve \cite{pensieve} relies on untraceable RL, and MPC \cite{mpc} relies on a rigid look-up table. (3) \bones considers future computational resources. While traditional scheduling algorithms may consider future bandwidth values, most of them only perform enhancement myopically within the real-time latency constraint. In contrast, \bones adopts a computational task buffer that not only enables enhancement options with better quality and higher latency but also makes the algorithm more robust to computational resource variations. (4) \bones also utilizes a bandwidth signal, both implicitly and explicitly. Though the basic version of \bones makes decisions based only on buffer occupancy, buffer level is a good indicator of bandwidth. After the startup stage, a lower buffer level implicitly indicates a drop in bandwidth, which then triggers \bones to be conservative in download bitrate. This behavior is similar to other throughput-based algorithms. Besides, the Auto-Tuning method we introduced in \cref{sec:ablation} explicitly utilizes the bandwidth signal to automatically adjust the hyper-parameters of \bones.  }


% todo: experiment?
\rev{It could be challenging to incorporate prediction into \bones while maintaining the theoretical guarantees brought by the Lyapunov optimization framework. However, it might be possible to bring it in via heuristic methods. We can extend the Auto-Tuning technique described in \cref{sec:ablation} to optimize the hyper-parameters of \bones based on the predicted bandwidth within a short time frame. This involves offline optimization of performance over all possible combinations over the hyper-parameter values and online selection of the corresponding settings.}


\textbf{Review \#69A:} \textit{Will the advantage of \bones still hold if there are changes in the trade-off among the three components of the composite QoE?}

% todo: popular qoe?
% It's true that different ABR or NES algorithms have different trade-offs among visual quality, quality oscillation, and rebuffering ratio.
\rev{We have illustrated the performance of \bones and all baselines in \cref{fig:nasall}. We find that the ABR baselines (dots) approximately form a curve, showing different trade-offs between visual quality and rebuffering ratio. NES baselines (triangles) form another curve on the right side of ABR baselines, improving their visual quality by using the additional computation power. In contrast, \bones deviates from them and lies in the bottom right corner of the figure, which means it achieves a better trade-off. The quality oscillation is denoted via error bars in the figure, and we observe that \bones also has a short bar (low oscillation). Therefore, \bones will outperform the baselines regardless of the specific trade-off settings in the composite QoE. It's also possible to adjust the optimization preference of \bones by tuning its hyper-parameters, as we have studied in \cref{sec:hyper}.
}

\textbf{Review \#69A:} \textit{Why maximizing $\Bar{s}$ in \cref{eq:smooth} is equivalent to minimizing the total rebuffering time?}

\rev{The total playback time equals the total video length plus the total rebuffering time because a video is either being played or frozen. To minimize the ratio of total rebuffering time over total playback time, we equivalently maximize their difference (total video length) over the total playback time. As explained in \cref{sec:objective} (Line 240-243), under the assumption of infinite video segments, we can approximate the total playback time by the total download time, because their gap is at most the finite time to drain the download buffer. Finally, \cref{eq:smooth} is derived by combining the total video length (enumerator) and the total download time (denominator).}

\textbf{Review \#69A:} \textit{Is $e_j$ needed in \cref{eq:smooth}?}

%  because the enhancement option $e_j$ will not affect the segment length $p$
\rev{Technically, it is not needed. It's kept there solely to match the format of $\Bar{u}$ defined in \cref{eq:utility}, which makes it more intuitive to merge terms when deriving \cref{eq:op}.}


% - The paper leaves many open aspects, including how to find a good balance and delivery of the enhancement models (e.g., content-aware vs content-agnostic), and several aspects left as future work (e.g., see end of conclusions).

% - It is unclear how realistic scenarios the system is evaluated on and the performance for the network-traces were not that convincing.  This leaves several question marks regarding to what extent the method would provide improvements in practice.

% - It is also unclear how practical the application would be (e.g., clients that have very poor connection but powerful computers ...) or whether the paper addresses a corner case.  In practice, I am worried that regular HAS/DASH will be good enough for most practical purposes.

% - It would be valuable to discuss the data requirements and potential limitations of BONES, especially in terms of data collection and computational resources needed for training (and who does the training when).  Some additional motivation may also be needed to motivate this use case in practice.  As of now, it is not obvious how and what incentives there are to deploy and integrate BONES into existing video streaming systems.

% Comments for authors
% --------------------
% Additional comments:
% - still unsure if I am okay with the first sentence ...
% - would be good to say what type of guarantees (in the abstract)
% - I did not like how many of the equations were introduced (e.g., equations (4) and (5).  I would have much rather seen them integrated into the text (e.g., as equations (6), (7), and (8)).
% + really like Figure 2
% - Please sort out y-axes numbering in Figure 6 (would not rotate these numbers)
% - Results in Figure 5 (and some others) may be made to be easier to
% - Would be nice to see more details/data regarding the increase in startup due to use of content-aware enhancement


\textbf{Review \#69B:} \textit{Is the evaluation test bed and network traces sufficiently realistic?}

\rev{The network traces we test over are realistic. We adopt the same testing dataset as BOLA \cite{bola, bola2}. Note that among all four sub-datasets, the FCC sub-datasets are also widely used by other studies \cite{nas, presr}, while the 3G and 4G sub-datasets are designed to test mobile cases. Beyond the simulation results, we also implemented a prototype system during the revision phase as described in \cref{sec:prototype}. Sufficient simulations and real-world experiments show that \bones consistently outperforms state-of-the-art baselines.}


\textbf{Review \#69B:} \textit{Is the application sufficiently practical? Does this paper only address a corner case (clients with poor networking connections but powerful computers)?}

\rev{ \bones is practically valuable in the following aspects. On the receiver side, \bones improves the worst-case user experience instead of addressing an insignificant corner case. During poor network connections, \bones provide an opportunity to leverage an additional dimension of computational resources for compensation, which will improve the worst-case user experience. The user may also intentionally lower the download bitrate to save bandwidth while still maintaining a satisfactory quality of experience by enabling \bones. On the sender side, \bones is appealing to video providers and uploaders. A video provider could stream lower-resolution videos and enable \bones on the client side, to cut its cost on bandwidth consumption while shifting the computational burden to the user device. The idea of neural-enhanced streaming can also benefit video uploaders. Existing studies \cite{livenas, nemo, neuroscaler} find that the bottleneck of live streaming is often the upstream bandwidth of uploaders. They then let uploaders only stream a lower-resolution video and deploy an enhancement module at the server or the client to upgrade its quality. \bones could also be extended to such live-streaming scenarios. We argue that eventually utilizing computational power in streaming via a scheduler like \bones will become more attractive and beneficial, as computational hardware and AI enhancement methods are developing rapidly. }

% todo: user intention to reduce bandwidth consumption

\textbf{Review \#69B:} \textit{Require more discussions about the training cost, including data collection, computational resources, and who and when to conduct the training.}

\rev{ \bones applies to arbitrary enhancement methods that trade computational resources for quality improvement, including those with no training phase and no training cost. Regarding those that require training such as super-resolution methods, we have discussed in \cref{sec:setting} that there are generally two types: content-agnostic and content-aware. Content-agnostic enhancement models are general models that treat all kinds of input videos equally. Video providers can directly use existing pre-trained models with no training cost, or train them offline before deployment. These models can be installed together with the video player onto the client device. In contrast, content-aware enhancement models are fine-tuned toward a specific video, sacrificing generalization ability for better quality. The video provider needs to prepare the target video, and then perform the fine-tuning which typically lasts for 10 minutes as analyzed in \cref{sec:overhead}. The training is also conducted offline, but the model can only be downloaded before a specific video is played. In between these two classes, some models are fine-tuned toward a category of videos. These models require the video provider to feed in training data but can be installed together with the video player.
}

\textbf{Review \#69B:} \textit{Require more discussions about the startup overhead in content-aware enhancement.}


\rev{We provide a comprehensive overhead analysis in \cref{sec:overhead}, where we discuss the training cost, download overhead, startup latency, and other relevant factors. We introduce the QuickStart trick to mitigate the startup latency of content-aware enhancement, providing a total of three prospective trade-off options between performance and overhead. We conclude that \bones offers significant QoE improvement with zero or little overhead.}


% - There have been more recent DRL solutions for scheduling problems. It would be helpful to use some of them as baselines. Right now the baselines are not the most recent algorithms (except only for PreSR).
% - My main concern of the paper would be about its contribution. First of all, the application of the Lyapunov optimization technique is quite standard. Thus, the theoretical contribution is limited. On the other hand, the experiments are done mainly by simulation (based on real traces). Although the comparison appears comprehensive, it would be better to have some test on real testbed.

% Comments for authors
% --------------------
% - There have been more recent DRL solutions for scheduling problems. It would be helpful to use some of them as baselines. Right now the baselines are not the most recent algorithms (except only for PreSR).
% - My main concern of the paper would be about its contribution. First of all, the application of the Lyapunov optimization technique is quite standard. Thus, the theoretical contribution is limited. On the other hand, the experiments are done mainly by simulation (based on real traces). Although the comparison appears comprehensive, it would be better to have some test on real testbed.

\textbf{Review \#69C:} \textit{Require more deep reinforcement learning (DRL) methods as baselines.}

% todo: implement one more abr?
\rev{There are indeed more state-of-the-art DRL methods. However, most of them are pure ABR methods without considering neural enhancement. A small portion of them consider neural enhancement but simply as a post-processing step with one option. We have represented this type of work by Pensieve with greedy enhancement. We intuitively argue that methods considering versatile enhancement methods will outperform them if the large decision space is well explored. We have already compared with PreSR, the only DRL method with multiple enhancement options to the best of our knowledge. It's beyond the scope of this paper to extend other DRL methods to the NES domain with various enhancement options, which requires non-trivial redesign in the state-action space, data preparation, and training.
}


\textbf{Review \#69C:} \textit{The theoretic contribution seems limited because the Lyapunov optimization technique is standard.}

%  And we manage to bypass the buffer constraint of enhancement by conception.
\rev{Our work is extended from BOLA, yet the extension is non-trivial. Firstly, the parallel-buffer system we proposed is critical to inherit the Lyapunov optimization framework and all its performance guarantees. In comparison, one may adopt a sequential buffer system where the segment is first downloaded into the download buffer, enhanced, and then stored in the enhancement buffer. Although this system's workflow is more intuitive, it poses difficulties in deriving performance bounds. Secondly, it is challenging to derive performance guarantees in a double-buffer system because the original BOLA heavily relies on the simplicity and properties of one single buffer. We rework all details and eventually introduce enhancement-related terms into the performance bound in \cref{the:perf}.}

\textbf{Review \#69C:} \textit{The practical contribution seems limited because experiments are only done by simulation.}

\rev{We have implemented a prototype system and conducted real-world experiments to verify the practical performance of \bones. More details can be found in \cref{sec:prototype}.}
